Ensuring High-Quality Randomness in Cryptographic Key Generation

The security of any cryptosystem relies on the secrecy of the system's secret keys. Yet, recent experimental work demonstrates that tens of thousands of devices on the Internet use RSA and DSA secrets drawn from a small pool of candidate values. As a result, an adversary can derive the device's secret keys without breaking the underlying cryptosystem. We introduce a new threat model, under which there is a systemic solution to such randomness flaws. In our model, when a device generates a cryptographic key, it incorporates some random values from an entropy authority into its cryptographic secrets and then proves to the authority, using zero-knowledge-proof techniques, that it performed this operation correctly. By presenting an entropy-authority-signed public-key certificate to a third party (like a certificate authority or SSH client), the device can demonstrate that its public key incorporates randomness from the authority and is therefore drawn from a large pool of candidate values. Where possible, our protocol protects against eavesdroppers, entropy authority misbehavior, and devices attempting to discredit the entropy authority. To demonstrate the practicality of our protocol, we have implemented and evaluated its performance on a commodity wireless home router. When running on a home router, our protocol incurs a 2.1x slowdown over conventional RSA key generation and it incurs a 4.4x slowdown over conventional EC-DSA key generation.

==> bg.tex <==
\section{Background}

When a device generates a cryptographic keypair,
it would ideally select its keys {\em uniformly at random}
from the space of all possible keys.
For example, in selecting a DSA keypair $\langle x, g^x \rangle$,
the device would pick each secret value $x \in \mathbb{Z}_q$
with probability $1/q$.

However, imperfect implementations or implementations that
do not have access to a good source of environmental randomness
might draw these secret values from some non-uniform distribution.
Consider a DSA key generation routine that relies on a very
weak random number generator---one that always returns 
the 16-bit process ID as its ``random'' value.
The probability that the key generation routine will pick 
a given secret $x$ value will be $2^{-16}$ for $x \in [0, 2^{16})$
and zero otherwise.
We use the terminology loosely, and will refer to such a value 
$x$ as having {\em low entropy}, {\em weak entropy}, or {\em weak randomness}.
We refer to value $x$ that is drawn from the uniform distribution
as having {\em strong entropy}.

In the RSA cryptosystem, the cryptographic secrets are the
primes $p$ and $q$ whose product is the RSA modulus $N$.
If a device generates $p$ and $q$ using a weak entropy source
(for example, by using a PRNG seeded with the process ID),
then it would be easy for an adversary to replay the prime
number



